Improving Emotional Support Delivery in Text-Based Community Safety Reporting Using Large Language Models

Emotional support is a crucial aspect of communication between community members and police dispatchers during incident reporting. However, there is a lack of understanding about how emotional support is delivered through text-based systems, especially in various non-emergency contexts. In this study, we analyzed two years of chat logs comprising 57,114 messages across 8,239 incidents from 130 higher education institutions. Our empirical findings revealed significant variations in emotional support provided by dispatchers, influenced by the type of incident, service time, and a noticeable decline in support over time across multiple organizations. To improve the consistency and quality of emotional support, we developed and implemented a fine-tuned Large Language Model (LLM), named dispatcherLLM. We evaluated dispatcherLLM by comparing its generated responses to those of human dispatchers and other off-the-shelf models using real chat messages. Additionally, we conducted a human evaluation to assess the perceived effectiveness of the support provided by dispatcherLLM. This study not only contributes new empirical understandings of emotional support in text-based dispatch systems but also demonstrates the significant potential of generative AI in improving service delivery.

==> 99_discussion.backup.tex <==
\section{Discussion}
In this section, we discuss the findings of this study and their connections to prior work and implications for future designs in the field of community safety risk reporting systems. 

\subsection{\textit{Hidden Facts}: Stakeholders'  Interactions through Text-based Reporting Systems}

We first focus on discussing what new understanding of user-dispatcher interaction in a text-based reporting system has been revealed by the results of this study. 


\textbf{Misaligned Perceptions on Risk Reporting Using Text-based Channels (RQ1)} 
Previous work identified that users are more likely to report an incident directly by dialing 911 when encountering emergencies and life-threatening incidents than using other channels of communication \cite{hughes2012evolving}.
Examples of emergency dispatch center training manuals also stated that callers under emergency situations should be routed to emergency lines immediately, reinforcing the role of these systems for high-severity incidents \cite{alameda_police_2020}. 
Our findings suggested that even under emergency situations, some users still choose to report through text-based systems. This is aligned with findings from recent studies about newly-emerged ICTs and their application for crisis management \cite{schraagen2011human} and incident reporting \cite{tabassum2022context}. 
Online text-based reporting may be perceived by users as more private and anonymous \cite{alarid2008citizens}, which might encourage users to report.
In addition, some users might use the text-based system if they are unable to speak, such as a user experiencing difficulty breathing or needing to report quietly. This type of situation has also been identified as a significant challenge for traditional call-taking systems \cite{neusteter2019911}. 
Our findings showed that under such situations, dispatchers were able to effectively communicate and offer both physical and mental support to users through the text-based communication channel. 
% Another possibility is that users in need of making a report might face linguistic barrier when talking to human dispatchers over the phone. Previous research has found that for international students, linguistic barrier has been a major concern for using some of the services provided by the institutes but only in English \cite{}. We also found a significant amount of tips from the initial data to be non-English tips. 

% difference in the information provided by users and that collected by dispatchers
Our findings from RQ1 also showed that although users tended to provide similar types of event information upfront (e.g., \textit{attacker}, \textit{victim}, \textit{location}, and \textit{time}), the types of information asked and elicited by dispatchers often differed across different event types. Meanwhile, the amount of information reported by users was also found to differ across event types. 
This suggests a difference between the information that is important from users' perception and that from safety organizations. This is also referred to as the "discrepancy between the perceived priority of concerns" by a previous study by Whalen et al.\cite{Observations_on_the_Display}. 
The implications of this finding are twofold: First, more information should be offered to align users' and dispatchers' perceptions on the details that are most important for responding to events. This can be accomplished by providing a well-designed event ontology with explicit explanations to help users and dispatchers communicate more effectively. Second, this conclusion emphasizes the significance of flexibility when developing new ICTs for the safety reporting area in order to capture information with multiple modalities for various sorts of occurrences. A flexible and adjustable event reporting system can help to bridge the gap between what information is most valuable to each stakeholder.

% \textbf{Proxy Reporting for Sensitive Event Types (RQ1)} 
% For some event types, users are observed to have reported on behalf of others. 
% \yiren{During interview with DPS staff, we learned that reports that are made on behalf of others are not counted as valid reports. However, this should not be the case.} 
% For those cases where the user reported emergency situations for their friends without obtaining permission, attempts should be made to collect contact information in order to follow up and remain connected with the reporter. 

% \textbf{Social Media in Safety Incident Reporting (RQ1)} Many hazardous events nowadays took place over social media and other online platforms. Social media have become an inevitable viable of safety incident either as location or means \todo{need citations here}, especially among the higher education community. 




\textbf{Inconsistency between Dispatchers' Responses (RQ2)}
According to prior works \cite{Observations_on_the_Display, feldman2021calming, paoletti2012operators}, 911 emergency line call-takers often have to handle callers' strong emotional displays in order to offer assistance and gather information. 
According to our RQ2 findings, we also observed similar behavior from users of the LiveSafe text-based reporting system. Using text, users were still observed to express emotional swings. We also identified several strategies used by administrators in response to users' emotions. 
In addition to strategies discussed in prior works\cite{Observations_on_the_Display, feldman2021calming}, we identified additional strategies specifically pertaining to expressions of emotional support from dispatchers. This resonates with previous works about the benefit of emotional support for crime victims \cite{DakofVictimsPerceptions}. 

However, we found that providing emotional support was not a standardized procedure consistently adopted by dispatchers under all circumstances. 
Our findings from RQ2 showed that not only does an organizational discrepancy exist in the practice of providing emotional support, but dispatchers' decisions on whether to provide emotional support were also found to be affected by profiles of users (i.e., anonymity and if reporting on behalf). Additionally, the responsiveness of dispatchers was seen to vary among event types.
This shed light on how responsiveness can be affected by administrators' perception of risk. Miscommunication and other undesirable outcomes might emerge from a mismatch in perceptions of risk on each side of the conversation \cite{garcia2015something}. ICTs can be utilized by agencies to improve the consistency in safety services to improve community trust \cite{SheenaExaminingTechnologyThat}.



% \textbf{Dispatcher Questioning Strategies (RQ2)} 
% Common practices of what-to-ask, combining with existing available guidelines and policies and theories; Do not ask multiple questions at once; Reports about emergency need to be handed to officers and handled immediately.

% Still, challenges also exist for dispatchers using text-based incident reporting systems. 

\textbf{The Myths of Emotional Support (RQ3)} 
% \textbf{Providing Emotional Support to Increase User Responsiveness (RQ3)} 
% \textbf{Difference in Perceived Urgency between Users and dispatchers (RQ3)} 
Prior research on text-based reporting systems has revealed the mismatch between what the safety departments expected to receive and what their community members actually reported \cite{ming2021examining}. This is due to a misalignment between the agency's restricted number of tip categories and how these categories are perceived by users. Users may be hesitant to report incidents as a result of this mismatch, lowering the level of service provided by safety agencies.
Previous research has emphasized the significance of service quality to emergency dispatch operations \cite{clawson2018litigation}. In this study, we discovered two additional organizational factors related to service quality that are associated specifically with users' responsiveness in reporting based on RQ3 findings: organizational emotional support and responsiveness, with users' responsiveness being positively associated with provided emotional support and administrator responsiveness.
The findings imply that administrators' behavior has a significant impact on community members' reporting responsiveness. This is consistent with other studies where it was discovered that users' reporting decisions were influenced by their level of trust in the effectiveness of the police \cite{goudriaan2006neighbourhood}. 

In the utility-cost model of users' reporting behavior, the decision of reporting is driven by users' estimation of benefits if a report is made and the cost of doing so. Prior works have suggested that victims who have low confidence in the efficacy of safety organizations may not value the benefits of reporting as highly \cite{baumer2002neighborhood, anderson2000code}. 
As a result, our study added empirical support to the idea that the responsiveness of users' reporting behavior may be influenced by safety agencies' service quality. To further quantify the process of users' reporting behavior, we propose to consider the reporting behavior as a sequential decision-making process, where methods such as the nested logit model may be adopted to better model and understand users' behavior \cite{lemp2010continuous}.
Another implication of our findings is that safety agencies can improve the quality of their services by providing emotional support and improving responsiveness to encourage users to report safety concerns and events.
 

% Our findings of RQ3 also revealed the difference between users' and dispatchers' responsiveness. As stated by Whalen et al. \cite{Observations_on_the_Display}, there exists a discrepancy between emergency line callers and call-takers in their perceived priority of concerns, \textit{``... Not surprisingly, then, an inherent tension exists between callers who regard their circumstances as both stressful and urgent, and call takers who somehow must manage the encounter and mobilize an organizational response ...''}. 


\subsection{Design Implications}
% \todo{This section needs more NLP works to backup the design feasibility}
In this section, we discuss the design implications yielded from this study's data analysis. 
% \todo{Why need a CA?}. \todo{use some papers from related works section 1, to motivate this} 
% Recent research has introduced AI-based systems to assist emergency dispatchers in decision-making \cite{chen2017machine, schenkel2018triage}.
Inspired by the conversational nature of text-based reporting systems, we identified the feasibility of incorporating an AI-enabled conversational agent (CA) into the user-dispatcher interaction during incident reporting. 
We focus on discussing the implications of our findings for introducing a \textit{\textbf{Human-CA Collaborative design}} that can augment the interaction between users and dispatchers in the context of text-based risk reporting systems. Specifically, we discuss the potential of using CAs to bootstrap responses for dispatchers from four perspectives: 
1) efficient incident information extraction; 
2) emotional intelligence; 
and 3) awareness of broader contexts. 

\textbf{CA for Automatic Safety Incident Information Collection} 
Our findings revealed that during a reporting conversation initiated by users with dispatchers, the common interaction process is that the dispatcher asks questions to collect information from the user’s response. We also discovered that dispatchers are inconsistent in 1) their responsiveness, 2) strategies used, and 3) whether or not they provide emotional support during this procedure.
Recent work explored the feasibility of using CA to help increase the effectiveness and efficiency of collecting evidential statements from both victims and witnesses \cite{minhas2022protecting}. Our findings also contributed to the growing body of evidence that a conversational agent tool can be created to increase communication consistency and efficiency by facilitating interactions between users and dispatchers~\cite{zheng2022ux}. The CA might improve service quality by supporting dispatchers in producing better reply messages, which would increase users' responsiveness. It could also directly increase reporting efficiency by automating the process of gathering essential event argument information. 
However, evidence collection systems proposed by prior studies \cite{minhas2022protecting, ku2008crime} either rely on rule-based methods or require a large amount of manually labeled training data. 
Future studies can adopt methods from recent NLP works from the domain of dialogue state tracking \cite{wu2019transferable, gao2019dialog, lee2021dialogue} and event argument extraction \cite{du2020event, lyu2021zero}. We also suggest future system design practitioners consider using pre-trained language models for more effective and robust event information extraction, by increasing the model's ability in domain adaptation and commonsense reasoning \cite{yang2019exploring}. 
% \todo{connect this to some NLP information-collecting dialogue system works ?}
% The CA should first check if an event is ongoing, if so collect location and suspect information. 

From our findings of RQ1, we observed several cases where the user was reporting on behalf of another person (the victim). Such reporting behaviors are often seen in situations where victims were unable or willing to report for themselves. This has been pointed out by previous studies in the context of crimes and safety incidents such as harassment \cite{matias2015reporting} and sexual abuse \cite{allnock2019snitches}. As an implication of this finding, we suggest that the CA should also be enabled to collect information about users' role in the incident, i.e. victim or witness. 
From the perspective of criminology, when encountering such incidents the victim might also refrain from reporting directly to the authority due to fear of possible retaliation by the offender\cite{ziegenhagen1977victims}. The system should be designed with support for non-victim users reporting on behalf or as a witness of the incident, to reduce the cost of reporting perceived by users. 
Thus it is important for the CA to recognize the role of the user in making the report. It would be beneficial to collect contact information from both the reporter and victim for further follow-ups. 

The found inconsistency in the responses from the dispatchers also points to the need for designs that will assist the dispatchers in incorporating more standardized question-asking strategies. 
% \todo{add dispatcher danger zone discussion}
Although not yet implemented by many safety organizations, clear and standardized protocols can be established as tools that can be used by dispatchers during incident handling \cite{clawson2018litigation}. A CA can be designed as a reminder and guide to help dispatchers follow a standardized question-asking protocol, thus reducing dispatchers' training cost \cite{casillo2020chatbot} and providing additional quality assurance.
We also discovered that dispatchers tended to have an inconsistent order in collecting event-related information when handling incidents that were more complicated. The CA can be designed to suggest what questions to ask next after analyzing user utterances and extracting useful event-related information, in order to assist dispatchers in questioning users.



\textbf{Enhancing CAs' Emotional Awareness} 
In the text-based reporting system context, the loss of emotional displays might have two-sided effects. First, from the organization's perspective, emotional displays can be helpful in understanding the situation and determining the best course of action. For example, a dispatcher might be able to use emotional displays to assess the severity of the incident. Without this knowledge, decision-making when providing support might be more difficult.
As opposed to that, the loss of emotional displays can increase the efficiency of the incident handling process by reducing time spent attempting to understand and handle the emotional state of the reporter, while also reducing the risk of making incorrect decisions based on users' inaccurate emotional cues, as in the case of Cukor vs. the city of Berkeley, where an officer was not dispatched because the caller spoke in a calm tone. The caller was ultimately killed by the intruder \cite{clawson2018litigation}. 

During our analysis for RQ2, we found that dispatchers tended to use generic languages with similar or sometimes even repetitive patterns to express emotional support for users. This includes circumstances where dispatchers try to express sympathy (e.g., "I'm sorry about what happened"), gratitude (e.g., "Thank you for using LiveSafe"), etc. Although these languages served as a gesture of caring and empathy, their generic and repetitive nature might be perceived by users as inauthentic, which can undermine the emotional support provided by the dispatchers \cite{kraak2017authentic}. Similar issues were also commonly found in interactions between human users and CAs. 
The lack of emotional awareness in CAs might lead to difficulty in establishing rapport with users and awkwardness during conversations \cite{minhas2022protecting, zheng2021pocketbot}. An emotion-aware CA can quickly gain users' trust and elicit more information from them \cite{lee2020hear}, thus significantly improving the efficiency of information gathering during safety incidents. 

Displaying emotional support can also help users to calm down during emergency situations. The CA should be emotionally aware of the user's reactions and attempt to calm the user if necessary, particularly in medical emergencies. The CA will be able to offer emotional support as well as information about relevant services to assist the caller.
Meanwhile, reporters' emotional information can be collected by the CA as a helpful source of information for the dispatchers to quickly understand the situation and further make incident handling decisions. The CA should also be aware of the minimal support that ought to be provided regardless of users' emotional displays and provide reminders to ensure the standard quality of support. 
% \yiren{As in the interview example, students fighting in front of bar}



% \textbf{Emotional Labor of Dispatchers (RQ2)}
Our findings of RQ2 also suggested an inconsistency in dispatchers' use of tone and responsiveness when handling users' tips. We also found a variety of strategies were adopted by dispatchers in providing emotional support to users. As discussed in Tracy et al.'s work \cite{tracy1998emotion}, 911 emergency call-takers often need to invest emotional labor and experience psychological burnout during the communication with callers. 
For dispatchers, having an emotionally aware CA can also help mitigate the emotional burnout and negative effect of emotional labor by providing suggested candidate messages and automating repetitive tasks, thus improving the efficiency and job satisfaction of dispatchers \cite{harvey2017can}. 
We argue that future studies to incorporate methods from recent related works on empathetic \cite{ma2020survey} and social chatbot \cite{shum2018eliza} to increase the emotional awareness of CA designs. 


% Improving users' trust in the dispatcher, social chatbot...


\textbf{Comprehending Conversational Context Information} 
% The CA should give regards to prior context information when providing responses. That is to say for different event types, the CA need to be capable of adapting tone and strategies based on situation. And for context, based on prior information provided by user, if the CA is aware of this information would make a different to the user in terms of dispatcher awareness, etc\todo{need citations here}. 
From our findings of RQ1, a case was observed where the dispatcher was found to have neglected contextual information initially provided by the user when reporting on behalf of the victim. Meanwhile, we discovered that most of the dispatchers' questions contained references that subtly alluded to contextual information expressed in earlier conversations (e.g., "Do you know who the someone was?", "do you know what dorms?"). Context information often plays a crucial role during conversational interactions of incident reporting.
Previous studies have shown that an increased awareness of contextual information during conversation boosts users' trust in the conversation agent \cite{loveys2020effect, rheu2021systematic}, and improves conversation effectiveness \cite{car2020conversational} and users' satisfaction \cite{purington2017alexa}. Our research indicates the value of context comprehension capabilities for the risk reporting conversation agent due to the discovered richness of contextual information during actual reporting conversations. The CA needs to be capable of adapting tone and strategies based on different situations according to conversation contexts.
% \todo{too weak, need more evidence to justify?}
Recent natural language generation (NLG) research has advanced itself in the direction of increasing the context awareness of task-oriented dialogue systems \cite{wu2020tod, liu2021context, kale2020template}. Future CA design could benefit from improved context awareness by incorporating techniques from related NLP works into the safety reporting domain.
